Triggering Multi-Hop Reasoning for Question Answering in Language Models using Soft Prompts and Random Walks

Despite readily memorizing world knowledge about entities, pre-trained language models (LMs) struggle to compose together two or more facts to perform multi-hop reasoning in question-answering tasks. In this work, we propose techniques that improve upon this limitation by relying on random walks over structured knowledge graphs. Specifically, we use soft prompts to guide LMs to chain together their encoded knowledge by learning to map multi-hop questions to random walk paths that lead to the answer. Applying our methods on two T5 LMs shows substantial improvements over standard tuning approaches in answering questions that require 2-hop reasoning.

==> data/metaqa <==
def prepare_metaqa_entry(
    line: str, prefix: str) -> Mapping[str, Union[str, Sequence[str]]]:
  r"""Prepares MetaQA question for training.

  MetaQA dataset is available here: https://github.com/yuyuz/MetaQA.
  Input line is expected to have question and set of answers. Question and
  answers should be separated by Tab. Different answers should be separated by
  |. Entity in the line should be inside of [].
  For example: 'what does [Laura Harring] act in\tMulholland Drive|Derailed'

  Args:
    line: line containing questions and answers.
    prefix: task prefix.

  Returns:
    Dictionary with input and answers. First answer is selected as target.
  """
  question, answers_line = line.strip().split('\t')
  entity_start = question.find('[')
  entity_end = question.find(']')
  entity = question[entity_start + 1:entity_end]
  question = question[:entity_start] + entity + question[entity_end + 1:] + '?'
  answers = answers_line.split('|')
  return {
      'inputs': prefix + question[0].upper() + question[1:],
      'targets': answers[0],
      'answers': answers
  }

==> tables/exp1results.tex <==
% Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table}[]
% \centering
% \resizebox{0.8\columnwidth}{!}{%
% \begin{tabular}{@{}lllll@{}}
% \toprule
% \textbf{Model} & \textbf{Size} & \textbf{Setup} & \textbf{1-hop} & \textbf{2-hop} \\ \midrule
% \multirow{4}{*}{\tfive{}} & \multirow{2}{*}{\textsc{large}} & PT & 4.36 & 4.47 \\
%  &  & FT & 6.24 & 10.03 \\ \cmidrule(l){2-5} 
%  & \multirow{2}{*}{\textsc{xxl}} & PT & 6.89 & 6.42 \\
%  &  & FT & 8.82 & 12.92 \\ \midrule
% \multirow{4}{*}{\ktfive{}} & \multirow{2}{*}{\textsc{large}} & PT & 6.30 &  \\
%  &  & FT & 22.73 & 11.19 \\ \cmidrule(l){2-5} 
%  & \multirow{2}{*}{\textsc{xxl}} & PT & 31.64 & 8.62 \\
%  &  & FT & 43.60 & 13.47 \\ \bottomrule
% \end{tabular}%
% }
% \caption{Results from prompt tuning and fine-tuning \tfive{} and \ktfive{} models on 2WikiMultiHopQA as well as the semi-automatically generated 1-hop QA dataset}
% \label{tab:exp1}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[h]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Setup}} & \multicolumn{2}{c}{\textbf{1-hop}} & \multicolumn{2}{c}{\textbf{2-hop}} \\ \cmidrule(l){3-6} 
 &  & \tfive{} & \ktfive{} & \tfive{} & \ktfive{} \\ \midrule
\multirow{2}{*}{\textsc{large}} & PT & 4.36 & \textbf{6.30} & 4.47 & \textbf{5.29} \\
 & FT & 6.24 & \textbf{22.73} & 10.03 & \textbf{11.19} \\ \midrule
\multirow{2}{*}{\textsc{xxl}} & PT & 6.89 & \textbf{31.64} & 6.42 & \textbf{8.62} \\
 & FT & 8.82 & \textbf{43.60} & 12.92 & \textbf{13.47} \\ \bottomrule
\end{tabular}%
}
\caption{Test set exact-match scores from prompt-tuning (PT) and fine-tuning (FT) \tfive{} and \ktfive{} models on 2WikiMultiHopQA \citep{ho-etal-2020-constructing} and its corresponding 1-hop questions.}
\label{tab:exp1}
\end{table}

==> tables/exp2results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.8\columnwidth}{!}{%
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Model} & \textbf{SPoT} & \textbf{Parse-then-Hop} & \textbf{Mixture} \\ \midrule
\ktl{} &  & 8.62 & 6.58\\
\ktxxl{} & 20.09 & 29.37 & 23.09 \\ \bottomrule
\end{tabular}%
}
\caption{Exact-match scores of methods that integrate random-walks in various ways on the 2-hop test set.}
\label{tab:exp2}
\vspace{-1em}
\end{table}

==> tables/mainexp.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[t!]
\centering
\resizebox{0.6\textwidth}{!}{%
\begin{tabular}{@{}lcccccccc@{}}
\toprule
\multirow{2}{*}{\textbf{Size}} & \multirow{2}{*}{\textbf{Hops}} & \multicolumn{2}{c}{\textbf{Fine-tuning}} & \multicolumn{2}{c}{\textbf{Prompt-tuning}} & \multirow{2}{*}{\textbf{\spot}} & \multirow{2}{*}{\textbf{\pth}} & \multirow{2}{*}{\textbf{\mixture}} \\ \cmidrule(lr){3-6}
 &  & T5 & \ktfive{} & T5 & \ktfive &  &  &  \\ \midrule
\multirow{2}{*}{\textsc{large}} & 1 & 6.24 & \textbf{22.73} & 4.36 & 6.30 & - & - & - \\
 & 2 & 10.03 & \textbf{11.19} & 4.47 & 5.29 & 7.22 & 8.62 & 6.58 \\ \midrule
\multirow{2}{*}{\textsc{xxl}} & 1 & 8.82 & \textbf{43.60} & 6.89 & 31.64 & - & - & - \\
 & 2 & 12.92 & 13.47 & 6.42 & 8.62 & 20.03 & \textbf{29.37} & 23.09 \\ \bottomrule
\end{tabular}%
}
\caption{Exact match (EM) scores achieved by various methods on 2WikiMultiHopQA \citep{ho-etal-2020-constructing} and its corresponding set of 1-hop questions. \spot{} \citep{vu-etal-2022-spot}, \pth, and \mixture{} are applied using \ktfive{}, and are only applicable for the main 2-hop dataset. Best scores for each model size and dataset (row-wise) are in \textbf{bold}.}
\label{tab:mainexp}
\vspace{-1em}
\end{table*}
